Why Do Pretrained Language Models Help in Downstream Tasks? An Analysis of Head and Prompt Tuning

Pretrained language models have achieved state-of-the-art performance when adapted to a downstream NLP task. However, theoretical analysis of these models is scarce and challenging since the pretraining and downstream tasks can be very different. We propose an analysis framework that links the pretraining and downstream tasks with an underlying latent variable generative model of text -- the downstream classifier must recover a function of the posterior distribution over the latent variables. We analyze head tuning (learning a classifier on top of the frozen pretrained model) and prompt tuning in this setting. The generative model in our analysis is either a Hidden Markov Model (HMM) or an HMM augmented with a latent memory component, motivated by long-term dependencies in natural language. We show that 1) under certain non-degeneracy conditions on the HMM, simple classification heads can solve the downstream task, 2) prompt tuning obtains downstream guarantees with weaker non-degeneracy conditions, and 3) our recovery guarantees for the memory-augmented HMM are stronger than for the vanilla HMM because task-relevant information is easier to recover from the long-term memory. Experiments on synthetically generated data from HMMs back our theoretical findings.

==> limitations.tex <==
\section{Limitations and societal impact}\label{sec:limitations}
\noindent{\bf Limitations.} The primary limitation of our work is that the analysis for prompt tuning has to be performed in an idealized setting where we assume the model processes the token embeddings in a very specific way, i.e., it treats the token embeddings as a vector describing token emission probabilities and performs message passing. Without making this assumption, it's extremely challenging to analyze the embeddings of the model directly, as this would require opening up the black box of the model. It seems unlikely that models pretrained in practice will entirely fit the assumptions we require for our prompt tuning analysis. However, we hope that our analysis can still provide insights into why prompt tuning might help, even with the assumptions it requires. 

Another limitation is that our results assume the model outputs the perfect conditional token probabilities, but this in practice we likely run into issues like model misspecification and suboptimal training. We believe it's possible for future work to use existing techniques to provide guarantees which account for errors in the probabilities predicted by the model. We decided to omit such analyses in order to obtain a cleaner first result.

\noindent{\bf Negative societal impact.} We don't foresee any negative impact of work, as our paper is theoretical and does not propose new algorithms.
